Getafix: Learning to Fix Bugs Automatically

Static analyzers help find bugs early by warning about recurring bug categories. While fixing these bugs still remains a mostly manual task in practice, we observe that fixes for a specific bug category often are repetitive. This paper addresses the problem of automatically fixing instances of common bugs by learning from past fixes. We present Getafix, an approach that produces human-like fixes while being fast enough to suggest fixes in time proportional to the amount of time needed to obtain static analysis results in the first place. Getafix is based on a novel hierarchical clustering algorithm that summarizes fix patterns into a hierarchy ranging from general to specific patterns. Instead of a computationally expensive exploration of a potentially large space of candidate fixes, Getafix uses a simple yet effective ranking technique that uses the context of a code change to select the most appropriate fix for a given bug. Our evaluation applies Getafix to 1,268 bug fixes for six bug categories reported by popular static analyzers for Java, including null dereferences, incorrect API calls, and misuses of particular language constructs. The approach predicts exactly the human-written fix as the top-most suggestion between 12% and 91% of the time, depending on the bug category. The top-5 suggestions contain fixes for 526 of the 1,268 bugs. Moreover, we report on deploying the approach within Facebook, where it contributes to the reliability of software used by billions of people. To the best of our knowledge, Getafix is the first industrially-deployed automated bug-fixing tool that learns fix patterns from past, human-written fixes to produce human-like fixes.

==> future_work.tex <==
\section{Future Work}\label{sec:future}
% technical

\paragraph{Fix interpolation.}
Seemingly insignificant differences in source code can result in significant changes in the AST representation.
As a result, fix patterns learnt by Getafix may be very sensitive to subtle variations of buggy code which it could otherwise fix.
For example, assume that Getafix knows the fix pattern wrapping call statement \code{h0.h1();} with a null-check for \code{h0} if it is the blamed variable.
The fix pattern's \before AST knows the method call expression \code{h0.h1()} as the child of an expression statement.
This pattern will not match a statement \code{g(x.f());} which has \code{x.f()} as the \textit{grandchild} of an expression statement (see last snippet of Example \ref{ex:selection_of_accepted_fixes}).

A fix pattern matching this example statement would be a slight variation of the original pattern.
We call such slight variations \textit{interpolations} of the original pattern.
Further AST variations like cast expressions (e.g. \code{((Foo)x).f()} or \code{(Foo)x.f()}) lead to combinatorial
explosion of interpolations required to reliably match all statements containing \code{h0.h1()}.

Getafix will learn any number of interpolations automatically when presented with a sufficient amount of samples in the training data.
However, it is possible that a fraction of bugs seen in the wild has an AST structure that did not occur in the training data.
One could manually assist Getafix by enumerating all fix pattern interpolations up to a desired maximum complexity (which requires language-specific knowledge) .
We have also considered introducing a \textit{descendant} relation in fix patterns in order to support representing above mentioned interpolations as a single fix pattern.
We did not investigate this idea further, for example it is unclear how/when the pattern mining step would opt for the descendant relation.


\paragraph{Machine learning.}
A variety of components of our pipeline could potentially benefit from integrating machine learning techniques:
For favoring special patterns for special circumstances, we currently rely on a combination of strong \before parts of a pattern and statistical reasoning to favour such strong patterns.
For example, this will ensure early return patterns that match on the return type (like returning \code{false} if the return type was \code{boolean}) are selected among more generic patterns.
This is a very strict and purely syntactic approach, which might not pick up on more subtle hints that could for example decide between early return patterns and wrapping patterns.
We have already experimented with training a classifier, hoping to be more sensitive to such subtleties.

\citet{Pradel2018DeepBugs} showed promising results in purely name-based bug detection.
It is likely that using a similar technique would benefit our learning and ranking phase, at the very least one could use word embeddings to capture the "flavor" of values that were substituted by holes.
For example, we have seen name-based indicators for when humans tend to fix Null Method Call warnings by wrapping the call with an if:
Method being wrapped are often logging calls, destruction (\code{release}, \code{close}), events (\code{on...}) or GUI updates (\code{focus}, \code{setDefault}), i.e. side effects that should have no further consequence on the control flow at the call site.
If the subject is \code{null} there is legitimately nothing to be done, rather than, for example, coming up with an alternative value for the subject.
Another potential application would be mimicking human intuition about the concrete return value to pick in case of an early return, for example \code{-1} for \code{indexOf}-like functions or \code{null} vs \code{""} for string functions.
We suspect that a name-based approach would be able to pick up those clues.

Getafix so far cannot learn change patterns within individual token values.
For example appending suffix \code{Async} to a method name could be represented by a pattern \edit{h0}{<h0 + "Async">} rather than \edit{h0}{h1} (which we would currently learn from two concrete rename edits \edit{get}{getAsync} and \edit{put}{putAsync}).
Getafix can represent either constant values or the act of copying a token from the \before tree precisely (via holes), but it can not perform simple computations on existing values to derive new values.
A strategy could be to use PROSE \cite{Polozov2015FlashMeta} during anti-unification:
When currently we would anti-unify a pair of tokens in the \after trees with a new unbound hole (if no existing hole matches exactly and can hence be reused),
we could instead attempt finding a function that can compute the token values based on existing holes.


\paragraph{Open patterns.}
Getafix generally does not attempt to apply "open" fix patterns, i.e. if a holes in the \after part is bound neither by the \before part nor the bug report.
With an appropriate method to instantiate the unbound holes, these fix patterns may prove useful as well.
For example, one could attempt instantiation using ingredients as done for example by \cite{Wen2018ContextAwarePG}.
In a more interactive context, for instance when suggesting fixes in an IDE, one could also let the developer choose an instantiation.


\paragraph{At Facebook.}
Getafix has helped us advance toward our goal of letting computers take care of routine bug-fixing work.
As we continue to refine our testing and verification tools, we expect Getafix will be able to prevent a larger portion of postdeployment failures.

We note that the fix patterns Getafix mines need not come only in response to Infer-related fixes.
Indeed, they can also come from fixes made during or in response to manual code review.
This additional source of fix patterns opens up the exciting possibility of automating repetitive code reviews.
In other words, a bug that has been flagged and remediated across the codebase multiple times in the past can be flagged automatically in a future code commit --- without a human needing to do it.

Getafix is part of our overall effort to build intelligent tools that rely on statistical analysis of large code corpora and the associated metadata.
Such tools have the potential to improve all aspects of the software development life cycle, including code discovery, code quality, and operational efficiency.
The insights we gain from Getafix will help us in building out and deploying additional tools in this space.

